Task-wise Sampling Convolutions for Arbitrary-Oriented Object Detection in Aerial Images

Arbitrary-oriented object detection (AOOD) has been widely applied to locate and classify objects with diverse orientations in remote sensing images. However, the inconsistent features for the localization and classification tasks in AOOD models may lead to ambiguity and low-quality object predictions, which constrains the detection performance. In this article, an AOOD method called task-wise sampling convolutions (TS-Conv) is proposed. TS-Conv adaptively samples task-wise features from respective sensitive regions and maps these features together in alignment to guide a dynamic label assignment for better predictions. Specifically, sampling positions of the localization convolution in TS-Conv are supervised by the oriented bounding box (OBB) prediction associated with spatial coordinates, while sampling positions and convolutional kernel of the classification convolution are designed to be adaptively adjusted according to different orientations for improving the orientation robustness of features. Furthermore, a dynamic task-consistent-aware label assignment (DTLA) strategy is developed to select optimal candidate positions and assign labels dynamically according to ranked task-aware scores obtained from TS-Conv. Extensive experiments on several public datasets covering multiple scenes, multimodal images, and multiple categories of objects demonstrate the effectiveness, scalability, and superior performance of the proposed TS-Conv.

==> Chap41.tex <==
In this section, extensive experiments are conducted on several AOOD datasets to evaluate the performance of TS-Conv comprehensively. First, the experimental conditions, including datasets, evaluation metrics, implementation details, etc., are introduced. Then, ablations experiments are designed to validate the effectiveness of each component of the TS-Conv model and to evaluate their performance quantitatively. The task-wise samplings, rotation-invariant feature extraction, dynamic label assignment, and other previously claimed issues in AOOD are discussed in detail. Forthermore, the scalability of TS-Conv on lightweight models and for multimodal data are evaluated. After that, comparative experiments with existing AOOD methods on the datasets covering different scenarios are given and analyzed. Besides, the extension of the proposed TS-Conv to improve the performance of lightweight AOOD models on embedded devices is further explored.

\subsection{Experimental Conditions}
\textbf{1) \textit{Experimental platforms.}} The experiments are performed on a server with an AMD 3950WX CPU, 128 GB memory, and four NVIDIA GeForce RTX 3090 GPU (24GB). In addition, the performance of the TS-Conv improved lightweight models are evaluated on embedded edge devices NVIDIA Jetson AGX Xavier and Jetson TX2.

\textbf{2) \textit{Datasets.}} To evaluate the performance of TS-Conv model more comprehensively, several public AOOD datasets are used, which cover different scenes, different shapes and categories of objects, and different data sources.

a) DOTAv1.0 \cite{xiaDOTALargeScaleDataset2018} dataset provides a widely used benchmark to evaluate the performance of AOOD methods in remote sensing scenes. It has more than 188,000 objects covering 15 categories in 2,806 images from $800\times800$ pixels to $4,000\times4,000$ pixels. Due to the huge size of remote sensing images, they are usually cropped into sub-images of $800\times800$ pixels with an overlap of 200 pixels on each dimension after being scaled to different sizes with the ratios of 0.5, 1.0, and 1.5 \cite{huang2021lo}. DOTAv2.0 \cite{li2020object} further expands the number of objects to 1,793,658 objects covering 18 categories. %The three new categories are 'Container-crane' (CC), 'Airport', and 'Helipad'.
 
b) HRSC2016 \cite{liu2017high} is a ship detection dataset consisting of 436 training images, 181 validation images, and 444 testing images from $300\times300$ pixels to $1500\times900$ pixels.

c) DIOR-R \cite{ding2021object,cheng2022anchor} dataset is an aerial AOOD datasets contains 190,288 objects covering 20 categories in 23,463 images with the size of $800\times800$ pixels. In the DIOR-R dataset, 5,862 images are used for training, 5,863 images are used for validation, and 11,738 images are used for testing. 

d) DroneVehicle \cite{sun2022drone} is an infrared-RGB vehicle detection datasets. After screening and pre-processing, 17,900 Infrared-RGB image pairs are used for training, 1,469 Infrared-RGB image pairs are used for validation, and 8980 Infrared-RGB image pairs are used for testing.

e) SSDD+ \cite{li2017ship} is a synthetic aperture radar (SAR) dataset for ship detection. It has 1,160 ship images including 2,456 instances collected from different sea conditions. The ratio of training, validation and testing images is 7:1:2.

\textbf{3) \textit{Evaluation metrics.}} The mean Average Precision (mAP) is adopted for evaluating the detection accuracy. The mAP with an IoU threshold of 50\% is represented as mAP$_{50}$. mAP$_{50:95}$ means calculating the mAP when the IoU threshold is 50\% to 95\% at every 5\% interval and then taking their mean as mAP$_{50:95}$. The speed is evaluated by frames per second (fps) and the computational complexity is evaluated by the floating point operations (FLOPs) for lightweight models.

\textbf{4) \textit{Implementation details.}}  The initial learning rate for training DOTA, DIOR-R, HRSC2016 and SSDD+ datasets is $5\times10^{-4}$, and the final learning rate is $1\times10^{-6}$. The optimizer for training the CNN model is stochastic gradient descent (SGD), and the learning rate scheduler is cosine decay. The weight decay and momentum are set as $5\times10^{-4}$ and 0.9, respectively. The batch size is 32 (8 images per GPU). The maximum training epoch for DOTA, DIOR-R, HRSC2016, DroneVehicle and SSDD+ datasets are 36, 150, 150, 50 and 150, respectively. The non-maximum suppression (NMS) threshold is 0.4. Random cropping, random flipping, random rotation and mixup strategies are employed for data augmentation.

\subsection{Ablation Experiments}
The results of the ablation experiments for different components of TS-Conv, including LS-Conv, CS-Conv with DCK, and DTLA, are presented in Table~\ref{table:2}. The anchor-free AOOD method GGHL \cite{huang2022general} is chosen as the baseline, and experiments are conducted on the most widely used AOOD dataset DOTA v1.0 \cite{xiaDOTALargeScaleDataset2018}. 

\textbf{1) Ablation experiments of each component.} First, as a control group, the shared-offset DCNs employed by RepPoints \cite{yang2019reppoints}, Oriented RepPoints \cite{li2022oriented}, etc., are introduced based on GGHL. This design has the same sampling positions for localization and classification features and maps these features to aligned locations. Although the above scheme somewhat enables more objects to be detected and improves the mAP$_{50}$ by 0.82, the improvement of the stricter metrics, i.e., mAP$_{75}$ and mAP$_{50:95}$, is slight. It implies that the model may relax its requirements for detection quality to accommodate two different tasks.
\begin{table*}[tp]
	\centering
	\renewcommand\arraystretch{1}
	\setlength{\tabcolsep}{2.5mm}{
		\caption{\label{table:2}
			{Ablation experiments of the proposed TS-Conv on the DOTAv1.0 dataset}}
		\resizebox{\textwidth}{!}{\setlength{\tabcolsep}{1mm}{
				\begin{tabular}{c|c|c|c|c|c|c|c|ccc}
					\hline\hline
					{\multirow{2}{*}{Methods}}     & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Decoupled \\ Head\end{tabular}} &\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Shared-offset \\ DCNs  \end{tabular}} &
					%					\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Independent \\ -offsets DCNs  \end{tabular}} &
					\multicolumn{3}{c|}{\begin{tabular}[c]{@{}c@{}}Task-wise DCNs \\ (TS-DCN) \end{tabular}}& \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Label \\ Assignment \end{tabular}} &  \multicolumn{3}{c}{mAPs on the DOTAv1.0 Dataset} \\ \cline{4-11}
					%Results(\%)
					& & & LS-Conv & CS-Conv & DCK & GGHL & DTLA & mAP$_{50}$ & mAP$_{75}$ & mAP$_{50:95}$ \\ \hline
					
					Baseline (GGHL \cite{huang2022general}) & $\checkmark$ & & & & & $\checkmark$ &  & 76.95 & 44.19 & 44.29 \\ \hline
					
					\begin{tabular}[c]{@{}c@{}}Shared-offset DCNs \\ (O-RepPoints \cite{li2022oriented})\end{tabular} & $\checkmark$ &  $\checkmark$ & & & & $\checkmark$ &  & 77.77 \tiny{(+0.82)} & 44.76 \tiny{(+0.57)} & 44.99 \tiny{(+0.70)} \\ \hline
					
					LS-Conv& $\checkmark$ & & $\checkmark$ & & & $\checkmark$ &  & 78.08 \tiny{(+1.13)} & 46.38 \tiny{(+2.19)} & 45.87 \tiny{(+1.27)} \\ \hline
					
					\begin{tabular}[c]{@{}c@{}} CS-Conv \end{tabular} & $\checkmark$ & & & $\checkmark$ &  & $\checkmark$ &  & 77.84 \tiny{(+0.89)} & 44.23 \tiny{(+0.04)} & 45.37 \tiny{(+1.08)}\\ \hline % \\ (Independent-offsets DCNs)$\bullet \; \blacktriangle$
					
					\begin{tabular}[c]{@{}c@{}}CS-Conv with DCK\end{tabular}& $\checkmark$ & & &  $\checkmark$ & $\checkmark$ & $\checkmark$ &  & 78.06 \tiny{(+1.11)} & 45.46 \tiny{(+1.27)} & 45.36 \tiny{(+1.07)}\\ \hline
					
					DTLA & $\checkmark$ & & & & & & $\checkmark$ & 77.95 \tiny{(+1.00)} & 46.10 \tiny{(+1.91)} & 45.38 \tiny{(+0.70)} \\ \hline
					
					TS-DCN & $\checkmark$ & & $\checkmark$ & $\checkmark$ & $\checkmark$ & $\checkmark$ &  & 78.13 \tiny{(+1.18)} & 46.59 \tiny{(+2.40)} & 46.09 \tiny{(+1.80)} \\ \hline
					
					\textbf{TS-Conv} & $\checkmark$ & & $\checkmark$ & $\checkmark$ & $\checkmark$ & & $\checkmark$ & \textbf{78.75 \tiny{(+1.80)}} & \textbf{46.60 \tiny{(+2.41)}} & \textbf{46.27 \tiny{(+1.98)}} \\ \hline
					\hline\hline
	\end{tabular}}}}\vspace{0.5em}
	\justifying{Note: Bold indicates the best result. 'Shared-offset DCN' represents that both branches of the decoupled head use DCN \cite{dai2017deformable} and their sampling offsets are shared as in the case of RepPoints \cite{yang2019reppoints} and Oriented RepPoints \cite{li2022oriented}.}
\end{table*}
\begin{figure}[!tp]
	\centering
	\epsfig{width=0.47\textwidth,file=7.pdf}
	\caption{Comparison of DTLA and GGHL label assignment strategies. Figs. (a-2)-(a-4) and (b-2)-(b-4) represent the positive candidate positions and their scores statically assigned by the GGHL strategy at three different scales, respectively. Figs. (a-5)-(a-7) and (b-5)-(b-7) represent the positive candidate positions and their scores dynamically assigned by the proposed DTLA strategy at three different scales, respectively. The closer the color is to red, the higher the score.}\label{fig:7}
\end{figure}
\begin{table}[!tp]
	\centering
	\renewcommand\arraystretch{1}
	\setlength{\tabcolsep}{1.8mm}{
		\caption{\label{table:3}
			{Evaluations of detection performance for different values of hyperparameters $T$ and $\vartheta$, and experiments of using DCK and random rotation data augmentation on the DOTAv1.0 dataset}}}
	\resizebox{0.48\textwidth}{!}{\setlength{\tabcolsep}{1.8mm}{
			\begin{tabular}{cc||cc||ccc}
				\hline\hline
				$T$ & mAP$_{50}$ & $\vartheta$ & mAP$_{50}$ & RandomRota & DCK & mAP$_{50}$ \\	
				\hline
				0.2 & 78.45 & 0.3 & \textbf{78.75} & $\checkmark$ & & 77.92 \\
				0.3 & \textbf{78.75} & 0.4 & 78.52 & & $\checkmark$ & 78.47\\
				0.4 & 78.60 & 0.5 & 78.50 & $\checkmark$ & $\checkmark$ & \textbf{78.75}\\
				\hline\hline
	\end{tabular}}}\vspace{0.5em}
	\justifying{Note: Bold indicates the best result. RadomRota represents using the random rotation data agumentation operation during the CNN training. When evaluating one variable, the other variables are fixed.}
\end{table}

Correspondingly, the proposed task-wise DCNs consisting of LS-Conv and CS-Conv are evaluated. With the introduction of LS-Conv, the mAP$_{75}$ is improved by 4.96\% (+2.19) compared to the baseline and 3.63\% (+1.62) compared to the shared-offset DCNs. The designed LS-Conv further improves the localization accuracy compared to the shared-offset DCNs by directly associating the convolutional sampling points with the OBB representation and embedding the spatial coordinates into the features. When only CS-Conv is used without LS-Conv, i.e., the sampling points of convolutions are just constrained in OBB, the mAP$_{50}$, mAP$_{75}$ and mAP$_{50:95}$ are also increased, but the improvement, especially for mAP$_{75}$, is minor. The bottleneck of this scheme is mainly in inaccurate localization. Because the spatial location coordinates of the OBB are explicit and essential features for the localization task, the convolutional sampling constraint of CS-Conv is vague for localization, although it is suitable for classification. In addition, since the objects in AOOD have richer orientation variations, performance improvements are also observed after replacing the convolutional kernel of CS-Conv with the designed DCK. Furthermore, when LS-Conv and CS-Conv are combined to obtain the TS-DCN scheme, significant performance gains are seen compared to using them alone as listed in Table~\ref{table:2}. The mAP$_{50}$, mAP$_{75}$ and mAP$_{50:95}$ are increased by 1.53\% (+1.18), 5.43\% (+2.40), and 4.06\% (+1.80), respectively. It illustrates that the LS-Conv and CS-Conv play complementary roles for each other. LS-Conv compensates for the lack of localization accuracy using only CS-Conv, while CS-Conv with DCK further improves detection performance.

Then, the performance of the two label assignment strategies, GGHL \cite{huang2022general} and the proposed DTLA, is evaluated. The proposed DTLA increases the mAP$_{50}$, mAP$_{75}$ and mAP$_{50:95}$ without introducing additional CNN structure and adding inference cost. Fig.~\ref{fig:7} shows the positive candidate positions selected by GGHL \cite{huang2022general} and DTLA for predicting objects. As seen in Fig.~\ref{fig:7}, there is a significant difference between the positive candidate positions dynamically selected by DTLA according to ${\tilde D}_{x,y}$ and the positions statically assigned by GGHL \cite{huang2022general} according to the Gaussian prior. The Gaussian peak position is not necessarily the optimal candidate position. It is more reasonable for DTLA to select the positive candidate positions adaptively according to different objects and training stages. 

Finally, the TS-Conv model combining the above components is obtained. Compared with the GGHL model, the mAP$_{50}$, mAP$_{75}$ and mAP$_{50:95}$ of TS-Conv are improved by 2.34\% (+1.80), 5.45\% (+2.41), and 4.47\% (+1.98). The improvement in mAP$_{75}$ and mAP$_{50:95}$ metrics representing higher detection quality is more pronounced. In general, the ablation experiments validate the effectiveness of each component in the proposed TS-Conv. In addition, Table~\ref{table:3} lists the experimental results of different hyperparameter settings. To obtain the best results, we set $T=0.3$ and $\vartheta=0.5$ in TS-Conv.

\textbf{2) Analysis of the IFS problem.} To more intuitively analyze the IFS problem faced by existing AOOD models like GGHL \cite{huang2022general}, Fig.~\ref{fig:8} visualizes the feature-sensitive regions of the localization and classification tasks. Fig.~\ref{fig:8} (a-1), (a-2), (b-1), (b-2), (c-1), (c-2), (d-1) and (d-2) show the feature sensitivity regions before using the proposed TS-Conv. The closer the color of the heatmap to red indicates that the model is more sensitive to the features in that region. From observing the feature sensitivity regions for various scenes and objects, it is obvious that the feature-sensitive regions of localization and classification tasks are significantly different. It is difficult for the existing schemes, such as decoupled-head used by CFC-Net \cite{ming2021cfc}, GGHL \cite{huang2022general}, etc., and shared-offset DCNs used by S$^2$ANet \cite{han2021align}, Oriented RepPoints \cite{li2022oriented}, etc., to take into account the respectively most sensitive features for different tasks. Correspondingly, Fig.~\ref{fig:8} (a-3), (a-4), (b-3), (b-4), (c-3), (c-4), (d-3) and (d-4) show the results of feature sensitivity regions after using the proposed TS-Conv. Sensitive features of different tasks located at different locations before input to TS-Conv are extracted and mapped to the same spatial location. The sensitive features of localization and classification are spatially aligned after TS-Conv's mapping. Then the optimal candidates are found among these spatially aligned features to predict the objects. It further demonstrates the effectiveness of the designed TS-Conv.
\begin{figure}[!t]
	\centering
	\epsfig{width=0.4\textwidth,file=8.pdf}
	\caption{Visualization of feature sensitivity regions. The closer the color is to red, the higher the sensitivity of the feature at this location. The figures in rows 1 and 3 (Figs. (a-1), (a-2), (b-1), (b-2), (c-1), (c-2), (d-1) and (d-2)) are the visualization results of feature sensitivity regions before using the designed TS-Conv. The figures in rows 2 and 4 (Figs. (a-3), (a-4), (b-3), (b-4), (c-3), (c-4), (d-3) and (d-4)) are the visualization results of feature sensitivity regions after using the designed TS-Conv.}\label{fig:8}
\end{figure}
\begin{figure}[!t]
	\centering
	\epsfig{width=0.4\textwidth,file=9.pdf}
	\caption{Visualization of features extracted by Dynamic circular kernel (DCK). Figs. (a-1)-(a-8) and Figs. (b-1)-(b-8) show the features extracted by convolutional kernels with different rotations in DCK, respectively. Figs. (a-9)-(a-12) and Figs. (b-9)-(b-12) show the DCK-extracted features of input images with different rotations, respectively.}\label{fig:9}
\end{figure}

\textbf{3) Analysis of orientation-robust features extracted by DCK.} Figs.~\ref{fig:9} (a-1)-(a-8) and Figs.~\ref{fig:9} (b-1)-(b-8) show the feature-sensitive regions of different oriented convolutional kernels in DCK (see details in Fig.~\ref{fig:5}), respectively. The different feature-sensitive regions indicate that the feature extraction is not robust to arbitrary orientations. Since objects' orientations in AOOD are more diverse than those in the ordinary OD, this problem further constrains the existing AOOD models' performance. Figs.~\ref{fig:9} (a-9) and (b-9) show the feature-sensitive regions of the designed DCK, which adjust the optimal orientation and weights of eight-oriented kernels according to different inputs adaptively. Furthermore, Figs.~\ref{fig:9} (a-9)-(a-12) and (b-9)-(b-12) show the feature-sensitive regions of DCK when the input images are rotated in different orientations. The results indicate that the feature-sensitive regions of DCK are robust to arbitrary-oriented inputs, which do not fluctuate significantly with the objects' rotations. In addition, the performance of using the random rotation data augmentation (RRDA) strategy and DCK are compared in Table~\ref{table:3}. The performance of the model using only DCK exceeds that of the model using only the RRDA strategy. As shown in Table~\ref{table:3}, when using both the RRDA strategy and DCK, the mAP$_{50}$ is 0.28 higher than that of using DCK only and 0.83 higher than that of using RRDA only. The performance further confirms the designed DCK's ability to enhance the model's robustness to extract features with arbitrary orientations.

\subsection{Experiments for the Scalability of TS-Conv}
\begin{table}[tbp]
	\centering
	\renewcommand\arraystretch{1}
	\setlength{\tabcolsep}{0.3mm}{
		\caption{\label{table:4}
			{Performance evaluation of the lightweight model using DTLA and TS-Conv-based knowledge distillation on the DOTAv1.0 dataset}}
		\resizebox{0.48\textwidth}{!}{\setlength{\tabcolsep}{0.3mm}{
				\begin{threeparttable}
					\begin{tabular}{c|ccccccc}
						\hline\hline
						\multirow{2}{*}{{Modules}} & \multirow{2}{*}{{mAP$_{50}$}}& \multirow{2}{*}{{\begin{tabular}[c]{@{}c@{}}Speed1\\ (fps)\end{tabular}}} & \multirow{2}{*}{{\begin{tabular}[c]{@{}c@{}}Speed2\\ (fps)\end{tabular}}} & \multirow{2}{*}{{\begin{tabular}[c]{@{}c@{}}Speed3\\ (fps)\end{tabular}}} & \multirow{2}{*}{{\begin{tabular}[c]{@{}c@{}}Speed4\\ (fps)\end{tabular}}}   & \multirow{2}{*}{{\begin{tabular}[c]{@{}c@{}}FLOPs\\ (G)\end{tabular}}} & \multirow{2}{*}{{\begin{tabular}[c]{@{}c@{}} Parameters\\  (MB)\end{tabular}}} \\ 
						{}& {} & {} & {}  & {} & {} & { }& { } \\
						%						{}& {} & {} & {}  & {} & {} & { }& { } \\
						\hline
						{LO-Det \cite{huang2021lo}} & {66.17}& {60.01} & {6.99}& {22.12} & 3.71 & {6.42} & {6.93}\\ \hline
						\begin{tabular}[c]{@{}c@{}} LO-Det \cite{huang2021lo} + GGHL \cite{huang2022general} \end{tabular}
						& \begin{tabular}[c]{@{}c@{}}71.26\\ \tiny{(+5.09)}\end{tabular} & 	\begin{tabular}[c]{@{}c@{}}62.07\\ \tiny{(+2.06)}\end{tabular} & 	\begin{tabular}[c]{@{}c@{}}7.68\\ \tiny{(+0.699)}\end{tabular}  & 	\begin{tabular}[c]{@{}c@{}}23.72\\ \tiny{(+1.60)}\end{tabular} & 	\begin{tabular}[c]{@{}c@{}}4.04\\ \tiny{(+0.33)}\end{tabular} & 	\begin{tabular}[c]{@{}c@{}}6.30\\ \tiny{(-0.12)}\end{tabular} & 	\begin{tabular}[c]{@{}c@{}}6.72\\ \tiny{(-0.21)}\end{tabular}   \\ \hline
						
						\begin{tabular}[c]{@{}c@{}}LO-Det \cite{huang2021lo} + DTLA \end{tabular}
						& \begin{tabular}[c]{@{}c@{}}73.36\\ \tiny{(+7.19)}\end{tabular} & 	\begin{tabular}[c]{@{}c@{}}62.07\\ \tiny{(+2.06)}\end{tabular} & 	\begin{tabular}[c]{@{}c@{}}7.68\\ \tiny{(+0.699)}\end{tabular}  & 	\begin{tabular}[c]{@{}c@{}}23.72\\ \tiny{(+1.60)}\end{tabular} & 	\begin{tabular}[c]{@{}c@{}}4.04\\ \tiny{(+0.33)}\end{tabular} & 	\begin{tabular}[c]{@{}c@{}}6.30\\ \tiny{(-0.12)}\end{tabular} & 	\begin{tabular}[c]{@{}c@{}}6.72\\ \tiny{(-0.21)}\end{tabular}   \\ \hline
						
						\begin{tabular}[c]{@{}c@{}} TS-Conv Lite \\ \footnotesize{(TS-Conv Distilled} \\ \footnotesize{LO-Det \cite{huang2021lo} + DTLA)} \end{tabular}
						& \begin{tabular}[c]{@{}c@{}} \textbf{73.96}\\ \textbf{\tiny{(+7.79)}}\end{tabular} & 	\begin{tabular}[c]{@{}c@{}}62.07\\ \tiny{(+2.06)}\end{tabular} & 	\begin{tabular}[c]{@{}c@{}}7.68\\ \tiny{(+0.699)}\end{tabular}  & 	\begin{tabular}[c]{@{}c@{}}23.72\\ \tiny{(+1.60)}\end{tabular} & 	\begin{tabular}[c]{@{}c@{}}4.04\\ \tiny{(+0.33)}\end{tabular} & 	\begin{tabular}[c]{@{}c@{}}6.30\\ \tiny{(-0.12)}\end{tabular} & 	\begin{tabular}[c]{@{}c@{}}6.72\\ \tiny{(-0.21)}\end{tabular}   \\
						
						\hline\hline
					\end{tabular}
	\end{threeparttable}}}}\vspace{0.5em}
	\justifying{Note: The unit G is Giga, which represents $1\times10^{9}$. The unit MB represents $1\times10^{6}$ bytes. Speed1, Speed2, Speed3 and Speed4 are the detection speed on the RTX 3090 GPU, NVIDIA Jetson TX2, Jetson AGX Xavier, and Jetson Nano, respectively. The inference speed only includes the network inference speed without post-processing.}
\end{table}
\begin{table}[tbp]
	\centering
	\renewcommand\arraystretch{1.2}
	\setlength{\tabcolsep}{1mm}{
		\caption{\label{table:5}
			{Performance evaluation of the proposed TS-Conv for multimodal images on the DroneVehicle dataset}}
		\resizebox{0.48\textwidth}{!}{\setlength{\tabcolsep}{1mm}{
				\begin{threeparttable}
					\begin{tabular}{c|c|c|cccccc}
						\hline\hline
						Methods & RGB & Infrared & car & freight car & truck & bus & van & mAP$_{50}$ \\
						\hline 
						\multirow{2}{*}{RetinaNet (OBB) [11]} &   $\checkmark$ &   & 67.50 & 13.72 & 28.24 & 62.05 & 19.26 & 38.16\\
						~ & & $\checkmark$& 79.86 & 28.05 & 32.84 & 67.32 & 16.44 & 44.90 \\
						\cdashline{1-9}[0.8pt/2pt]
						\multirow{2}{*}{Faster R-CNN (OBB) [11]} &  $\checkmark$ &  & 67.88 & 26.31 & 38.59 & 66.98 & 23.20 & 44.59\\
						~ & & $\checkmark$& 88.63 & 35.16 & 42.51 & 77.92 & 28.52 & 54.55 \\
						\cdashline{1-9}[0.8pt/2pt]
						\multirow{2}{*}{Faster R-CNN (Dpool) [11]} &  $\checkmark$ &   & 68.23 & 26.40 & 38.73 & 69.08 & 26.38 & 45.76 \\
						~ & & $\checkmark$& 88.94 & 36.79 & 47.91 & 78.28 & 32.79 & 56.94 \\
						\cdashline{1-9}[0.8pt/2pt]
						\multirow{2}{*}{Mask R-CNN [11]} &  $\checkmark$ &   & 68.23 & 26.40 & 38.73 & 69.08 & 26.38 & 45.76 \\
						~ & & $\checkmark$& 88.94 & 36.79 & 47.91 & 78.28 & 32.79 & 56.94 \\
						\cdashline{1-9}[0.8pt/2pt]
						
						\multirow{2}{*}{Cascade Mask R-CNN [11]} &  $\checkmark$ &   & 68.00 & 27.25 & 44.67 & 69.34 & 29.80 & 47.81 \\
						~ & & $\checkmark$& 81.00 & 38.97 & 47.18 & 79.32 & 33.00 & 56.96 \\
						\cdashline{1-9}[0.8pt/2pt]
						
						\multirow{2}{*}{Hybrid Task Cascade [11]} &  $\checkmark$ &   & 67.89 &27.22 &44.55 &70.22 &28.61 &47.70  \\
						~ & & $\checkmark$& 88.57 & 42.85 &47.71 &79.46 &34.16 &58.55 \\
						\cdashline{1-9}[0.8pt/2pt]
						
						\multirow{2}{*}{RoITransformer [11]} &  $\checkmark$ &   & 68.13& 29.08& 44.17& 70.55& 27.64 &47.91  \\
						~ & & $\checkmark$& 88.85& 41.49& 51.53& 79.48& 34.39& 59.15 \\
						\cdashline{1-9}[0.8pt/2pt]
						
						\multirow{2}{*}{ReDet [11]} &  $\checkmark$ &   & 69.48 &31.46 &47.87 &77.37 &29.03 &51.04  \\
						~ & & $\checkmark$& 89.47 &42.82 &53.95 &79.89 &36.56 &60.54 \\
						\cdashline{1-9}[0.8pt/2pt]
						
						\multirow{2}{*}{Gliding Vertex [11]} &  $\checkmark$ &   & 75.77& 33.75& 46.08& 68.05& 38.72& 52.48  \\
						~ & & $\checkmark$& 89.15 &42.95 &59.72 &78.75 &43.88 &62.89 \\
						\cdashline{1-9}[0.8pt/2pt]
						
						\multirow{2}{*}{GGHL } &  $\checkmark$ &   & 89.95 & 47.19 & 65.67 & 91.66 & 44.84 & 67.86  \\
						~ & & $\checkmark$& 94.32 & 53.45 & 64.63 & 90.85 & 51.38 & 70.93 \\
						\cdashline{1-9}[0.8pt/2pt]
						
						UA-CMDet [11] &  $\checkmark$ & $\checkmark$  & 87.51 &46.80 &60.70 &87.08 &37.95 & 64.01  \\
						\cdashline{1-9}[0.8pt/2pt]
						
						\hline\hline
					\end{tabular}
	\end{threeparttable}}}}\vspace{0.5em}
	\justifying{Note: The testing image size is 800 $\times$800 pixels. The TS-Conv$^*$ represents that it not only samples the features of different tasks separately, but also samples the features of different modalities.}
\end{table}

\textbf{1) Scalability of TS-Conv on lightweight models.} Although TS-Conv improves detection performance and robustness, the introduction of DCNs also brings additional computational burdens compared to the baseline model GGHL \cite{huang2022general}. For the benefits of TS-Conv to be applied in the lightweight model, the experiments on different embedded devices are designed and validated, as listed in Table~\ref{table:4}. The lightweight AOOD model LO-Det \cite{huang2021lo} is chosen as the baseline. First, the anchor-based label assignment strategy of LO-Det is improved to GGHL and the proposed DTLA for comparison. The results in Table~\ref{table:4} demonstrate that using the proposed dynamic label assignment strategy DTLA further improves the performance of the lightweight model by 2.95\% (+2.10) without losing model inference efficiency and increasing model complexity compared to using the static label assignment strategy GGHL. Second, the idea of knowledge distillation is adopted to make DTLA take full advantage of the task-wise sensitive features learned by TS-Conv without complicating the lightweight model structure. The LO-Det+DTLA is utilized as the student model, and the TS-Conv is used as the teacher model. The AOOD knowledge distillation method DKED \cite{huang2022extracting} is employed to guide the student model to learn the task-wise features of TS-Conv. The model obtained from this scheme is denoted as TS-Conv Lite. The results show that Ts-Conv Lite's performance is further improved without additional inference cost. TS-Conv Lite's mAP$_{50}$ improves 11.77\% (+7.79) compared to the baseline model with fewer model parameters and faster inference because it does not rely on anchor boxes.

\begin{figure}[tp]
	\centering
	\epsfig{width=0.48\textwidth,file=10.pdf}
	\caption{Visualization results of TS-Conv on the DroneVehicle dataset. Figs. (a-1)-(a-3) show the object detection results of RGB-Infrared multimodal image pairs under different lighting conditions. Figs. (b-1)-(b-4) show the feature sensitivity regions of different modalities and different tasks for RGB-Infrared multimodal image pairs.}\label{fig:10}
\end{figure}
\begin{figure}[!tp]
	\centering
	\epsfig{width=0.48\textwidth,file=11.pdf}
	\caption{Visualization results of TS-Conv on the DOTA dataset.}\label{fig:11}
\end{figure}

\textbf{2) Scalability of TS-Conv for multimodal data.} The effectiveness of the proposed TS-Conv for multimodal data is evaluated on the multimodal AOOD dataset DroneVehicle \cite{sun2022drone}. The results are shown in Table~\ref{table:5} and Fig.~\ref{fig:10}. The performance of the proposed TS-Conv and the baseline model GGHL are evaluated on RGB images, infrared images, and RGB-infrared image pairs, respectively. The results demonstrate that TS-Conv has improved performance compared with GGHL in all three groups of experiments. It illustrates the effectiveness of TS-Conv on multimodal data and demonstrates the merits of TS-Conv for improving the accuracy of oriented bounding boxes.

TS-Conv has discussed the differences in task-wise feature-sensitive regions, furthermore, the differences in modality-wise feature-sensitive regions are analyzed here. Figs.\ref{fig:10} (b-1)-(b-4) show the differences between task-wise and modality-wise features for RGB-Infrared image pairs. RGB images contain richer color and texture features but are more susceptible to lighting conditions. Infrared images highlight objects in low light conditions but lack more detailed features. Therefore, TS-Conv is extended to sample modality-wise features separately along the lines of "separate sampling and aligned mapping". This model is denoted as TS-Conv$^*$. The results in Table~\ref{table:5} reflect the effectiveness of the modality-wise samplings strategy for further improving the detection performance on the multimodal dataset. In the future, this problem is expected to be explored in more depth. In addition, experiments with lightweight models are also conducted to verify the scalability of TS-Conv on multimodal data.

\subsection{Comparison Experiments}
In this subsection, the performance of the proposed TS-Conv and state-of-the-art methods is compared on several datasets, including DOTA \cite{xiaDOTALargeScaleDataset2018,li2020object}, DIOR-R \cite{cheng2022anchor}, HRSC2016 \cite{liu2017high}, SSDD+ \cite{li2017ship}, SKU-110KR \cite{pan2020dynamic}, etc.
\begin{table*}[tp]
	\centering
	\renewcommand\arraystretch{1}
	\setlength{\tabcolsep}{0.43mm}{
		\caption{\label{table:6}
			{Comparative experiments on the DOTAv1.0 dataset}}
		\resizebox{\textwidth}{!}{\setlength{\tabcolsep}{0.43mm}{
				\begin{threeparttable}
					\centering
					\begin{tabularx}{\textwidth}{c|c|c|c|ccccccccccccccc|c|c}
						\hline\hline
						\multirow{2}{*}{Methods}                                  & \multirow{2}{*}{Backbone} & \multirow{2}{*}{Stage}& \multirow{2}{*}{Anchor} & \multirow{2}{*}{PL} & \multirow{2}{*}{BD} & \multirow{2}{*}{BR} & \multirow{2}{*}{GTF} & \multirow{2}{*}{SV} & \multirow{2}{*}{LV} & \multirow{2}{*}{SH} & \multirow{2}{*}{TC} & \multirow{2}{*}{BC} & \multirow{2}{*}{ST} & \multirow{2}{*}{SBF} & \multirow{2}{*}{RA} & \multirow{2}{*}{HA} & \multirow{2}{*}{SP} & \multirow{2}{*}{HC} & \multirow{2}{*}{mAP$_{50}$} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Speed\\ (fps)\end{tabular}} \\
						& &  &  &  &  &  &  & &  &  & &  &  & & & & & &  &  \\ \hline
						%			\multicolumn{20}{l}{\textit{Single-Stage Methods:}} \\ \cdashline{1-20}[0.8pt/2pt]
						ROI Trans. \cite{ding2019learning} & R-101 & Two & AB & 88.53& 77.91 & 37.63& 74.08 & 66.53& 62.97  & 66.57& 90.50& 79.46& 76.75& 59.04  & 56.73& 62.54  & 61.29 & 55.56& 67.74& 7.80 \\
						SCRDet \cite{yangSCRDetMoreRobust2019} & R-101 & Two & AB & 89.98& 80.65 & 52.09& 68.36 & 68.36 & 60.32 & 72.41 & 90.85& 87.94& 86.86 & 65.02 & 66.68  & 66.25  & 68.24  & 65.21  & 72.61  & 9.51\\
						RSDet \cite{qian2019learning} & R-101 & Two & AB & 89.80 & 82.90  & 48.60& 65.20& 69.50 & 70.10 & 70.20 & 90.50  & 85.60 & 83.40 & 62.50 & 63.90& 65.60 & 67.20& 68.00  & 72.20 & -  \\	
						Gliding Vertex \cite{xu2020gliding} & R-101 & Two & AB & 89.64 & 85.00 & 52.26 & 77.34 & 73.01 & 73.14 & 86.82 & 90.74& 79.02  & 86.81 & 59.55  & \textbf{70.91} & 72.94 & 70.86 & 57.32 & 75.02 & 13.10 \\			
						CSL \cite{yang2020arbitrary}& R-152 & Two & AB & \textbf{90.25}  & 85.53 & 54.64  & 75.31 & 70.44  & 73.51 & 77.62 & 90.84 & 86.15 & 86.69  & 69.60 & 68.04 & 73.83 & 71.10 & 68.93 & 76.17 & 8.89 \\			
						Oriented R-CNN \cite{xie2021oriented} & R-50 & Two & AB & 89.84 & 85.43&  \textbf{61.09} & 79.82 & 79.71&  \textbf{85.35} & 88.82 & 90.88&  86.68 & 87.73 & 72.21 & 70.80 & \textbf{82.42} & 78.18&  74.11 & \textbf{80.87}
						& 8.10\\
						\hline
						O$^2$-DNet \cite{wei2020oriented} & H-104 & One & AF & 89.31 & 82.14  & 47.33  & 61.21  & 71.32 & 74.03 & 78.62& 90.76 & 82.23 & 81.36  & 60.93 & 60.17 & 58.21 & 66.98 & 61.03 & 71.04 & - \\
						BBAVectors \cite{yi2020oriented} & R-101& One & AF & 88.35& 79.96& 50.69 & 62.18& 78.43& 78.98 & 87.94 & 90.85 & 83.58& 84.35& 54.13& 60.24 & 65.22 & 64.28 & 55.70 & 72.32 & 18.37 \\
						%			DRN \cite{pan2020dynamic} & H-104 & One & AF & 89.71 & 82.34 & 47.22 & 64.10 & 76.22 & 74.43 & 85.84 & 90.57 & 86.18& 84.89& 57.65& 61.93 & 69.30 & 69.63 & 58.48 & 73.23 & - \\	
						CFC-Net \cite{ming2021cfc}& R-50  & One & AB & 89.08 & 80.41 & 52.41 & 70.02 & 76.28 & 78.11 & 87.21 & 90.89 & 84.47  & 85.64 & 60.51 & 61.52 & 67.82 & 68.02 & 50.09 & 73.50 & 17.81 \\
						RIDet \cite{ming2021optimization} & R-101 & One & AB & 88.94 & 78.45 & 46.87 & 72.63 & 77.63 & 80.68 & 88.18 & 90.55 & 81.33 & 83.61 & 64.85 & 63.72 & 73.09 & 73.13 & 56.87 & 74.70 & 13.36\\
						GGHL \cite{huang2022general} & D-53 & One & AF & 89.74 & 85.63  & 44.50  & 77.48 & 76.72  & 80.45 & 86.16 & 90.83 & \textbf{88.18} & 86.25 & 67.07 & 69.40 & 73.38 & 68.45 & 70.14 & 76.95 & 42.30 \\					
						PolarDet \cite{zhao2021polardet} & R-101 & One & AF & 89.65& \textbf{87.07} &48.14 &70.97 &78.53 &80.34& 87.45& 90.76 &85.63 &86.87 &61.64 &70.32& 71.92& 73.09& 67.15& 76.64 & 25.00 \\
						GWD \cite{yang2021rethinking} & R-152 & One & AB & 86.96 & 83.88 & 54.36 & 77.53 & 74.41 & 68.48 & 80.34 & 86.62 & 83.41 & 85.55 & \textbf{73.47} & 67.77 & 72.57 & 75.76 & 73.40 & 76.30 & 13.86 \\
						KFIoU \cite{yang2022kfiou} & R-152 & One & AB &89.46 &85.72 &54.94 &80.37 &77.16 &69.23 &80.90 &90.79 &87.79 &86.13 &73.32 &68.11 & 75.23 & 71.61 & 69.49 & 77.35 & 13.79 \\ \hline
						R$^3$Det \cite{yang2019r3det} & R-152 & Refine & AB & 89.80 & 83.77 & 48.11 & 66.77 & 78.76 & 83.27 & 87.84 & 90.82& 85.38 & 85.51& 65.67 & 62.68 & 67.53 & 78.56 & 72.62 & 76.47  & 12.39 \\
						\cdashline{1-21}[0.8pt/2pt]	 
						\multirow{2}{*}{S$^2$A-Net \cite{han2021align}} & R-50 & Refine & AB  & 89.07  & 82.22 & 53.63  & 69.88 & 80.94  & 82.12 & 88.72  & 90.73 & 83.77 & 86.92 & 63.78 & 67.86 & 76.51 & 73.03& 56.60 & 76.38 & 17.60\\
						~ & R-101 & Refine & AB & 88.89 & 83.60 & 57.74 & \textbf{81.95} & 79.94 & 83.19  & \textbf{89.11} & 90.78& 84.87 & \textbf{87.81} & 70.30 & 68.25 & 78.30 & 77.01 & 69.58 & 79.42 & 13.79\\
						\cdashline{1-21}[0.8pt/2pt]
						\multirow{2}{*}{G-Rep \cite{hou2022g}} & R-50 & Refine & AF & 87.76 &81.29 &52.64 &70.53 &80.34 &80.56 &87.47 &90.74 &82.91 &85.01 &61.48& 68.51 &67.53 &73.02 &63.54 &75.56 & 14.74 \\
						~ & RX-101 & Refine & AF & 88.98 &79.21 &57.57 &74.35 &81.30 &85.23 &88.30 &90.69& 85.38 &85.25 &63.65 &68.82 &77.87 &78.76& 71.74 & 78.47 & - \\
						\cdashline{1-21}[0.8pt/2pt]
						\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Oriented \\ RepPoints \cite{li2022oriented}\end{tabular}} & R-50 & Refine & AF & 87.02 & 83.17  & 54.13  & 71.16 & 80.18  & 78.40 & 87.28 & \textbf{90.90} & 85.97 & 86.25 & 59.90 & 70.49 & 73.53 & 72.27 & 58.97 & 75.97 & 16.10 \\
						~ & R-101 & Refine & AF & 89.53 & 84.07  & 59.84 & 71.76 & 79.95 & 80.03 & 87.33 & 90.84 & 87.54 & 85.23 & 59.15 & 66.37 & 75.23 & 73.75 & 57.23 & 76.52 & 14.23 \\
						~ & Swin-T & Refine & AF & 88.72 & 80.56  & 55.69  & 75.07 & \textbf{81.84}  & 82.40 & 87.97 & 90.80 & 84.33 & 87.64 & 62.80 & 67.91 & 77.69 & \textbf{82.94} & 65.46 & 78.12 & -\\
						\hline
						\textbf{TS-Conv} & D-53 & Refine & AF & 89.86 & 87.05 & 49.12 & 74.01 & 78.97 & 81.28 & 88.24 & 90.77 & 86.85 & 87.24 & 71.87 & 69.88 & 77.01 & 70.43 & \textbf{78.63} & 78.75 & 23.23 \\
						
						\textbf{TS-Conv Lite} & Mobile2 & One & AF & 89.08 & 84.20 & 38.08 & 74.47 & 77.03 & 75.40 & 86.50 & 90.84 & 79.44 & 85.63 & 59.33 & 66.51 & 67.03 & 67.73 & 68.12 & 73.96 & \textbf{62.07} \\
						
						\hline\hline
					\end{tabularx}
	\end{threeparttable}}}}\vspace{0.5em}
	\justifying{Note: Bold font indicates the best results. The backbone networks R50, R-101, R-152, H-104, D-53, RX-101, Swin-T, and Mobile2 represent the ResNet50 \cite{he2016deep}, ResNet101 \cite{he2016deep}, ResNet152 \cite{he2016deep}, Hourglass104 \cite{zhou2019objects}, DarkNet53 \cite{redmonYOLOv3IncrementalImprovement2018}, ResNeXt101 \cite{xie2017aggregated}, Swin Transformer Tiny \cite{liu2021swin}, and MobileNetv2 \cite{sandler2018mobilenetv2}, respectively. 'One', 'Two', 'Refine' represent the one-stage method, two-stage method and refine-stage method, respectively. 'AF' represents anchor-free methods, and 'AB' represents anchor-based methods. The inference speed only includes the network inference speed (batch size=1) on an RTX 3090 GPU. When testing other methods, their open source codes are used. Since the deep learning frameworks are different, there may be slight relative errors in the test speed. The speed of some methods could not be tested due to the available codes, which is indicated by “-”. Regarding some methods, we have tried our best but failed to reproduce the results shown in their original papers, so the best results reported by them are listed in the Table.} 
\end{table*}
\begin{table}[tp]
	\centering
	\renewcommand\arraystretch{1}
	\setlength{\tabcolsep}{1.3mm}{
		\caption{\label{table:7}
			{Comparative performance of different methods on DOTAv1.0, DOTAv1.5, and DOTAv2.0 datasets}}
		\resizebox{0.48\textwidth}{!}{\setlength{\tabcolsep}{1.5mm}{
				\begin{threeparttable}	
					\begin{tabular}{c|ccc}
						\hline\hline
						Methods   & 
						\begin{tabular}[c]{@{}c@{}}mAP$_{50}$@v1.0\end{tabular}
						& 						\begin{tabular}[c]{@{}c@{}}mAP$_{50}$@v1.5\end{tabular} & 						\begin{tabular}[c]{@{}c@{}}mAP$_{50}$@v2.0\end{tabular} \\ \hline
						RetinaNet OBB \cite{linFocalLossDense2017} & 66.28 & 59.16 & 46.68 \\
						Mask R-CNN \cite{ding2021object} & 70.71 & 62.67 & 49.47 \\
						Cascade Mask R-CNN \cite{ding2021object} & 70.96 & 63.41 & 50.04 \\
						Hybrid Task Mask \cite{ding2021object} & 71.21 & 63.40 & 50.34 \\
						Faster R-CNN OBB \cite{renFasterRCNNRealTime2017a} & 69.36 & 62.00 & 47.31 \\
						Faster R-CNN OBB + Dpool \cite{ding2021object} & 70.14 & 62.20 & 48.77 \\		
						Faster R-CNN H-OBB \cite{ding2021object} & 70.11 & 62.57 & 48.90 \\	
						Faster R-CNN OBB + RT \cite{ding2021object} & 73.76 & 65.03 & 52.81 \\						
						\hline
						GGHL \cite{huang2022general} (Baseline) & 73.98  & 68.92 & 57.17 \\ 
						\textbf{TS-Conv} & \textbf{75.04 \tiny{(+1.06)}} & \textbf{71.18 \tiny{(+2.86)}} & \textbf{59.77 \tiny{(+2.60)}}   \\
						\hline\hline
					\end{tabular}
	\end{threeparttable}}}}\vspace{0.5em}
	\justifying{Note: Bold font indicates the best results. In order to make a fair comparison with the methods in the DOTAv2.0 benchmark \cite{ding2021object}, the experiments above do not use data augmentation and other tricks like these comparison methods. $mAP_{50}$@v1.0, $mAP_{50}$@v1.5, and $mAP_{50}$@v2.0 denote the results on the DOTAv1.0, DOTAv1.5, and DOTAv2.0 datasets \cite{li2020object}, respectively.}
\end{table}

\textbf{1) Comparison experiments on the DOTA datasets.} Table~\ref{table:6} provides the performance comparison results of the different methods on the most widely used AOOD dataset DOTAv1.0. The experimental results show that the performance and speed of the proposed TS-Conv outperform most of the AOOD methods (mAP$_{50}$=78.75), further validating the effectiveness of TS-Conv. Although the performance of TS-Conv is slightly lower than that of the two-stage method Oriented R-CNN \cite{xie2021oriented} and the refine-stage method S$^2$ANet (with the larger backbone ResNet-101) \cite{han2021align}, the detection speed of TS-Conv is much faster than those of Oriented R-CNN \cite{xie2021oriented} and S$^2$ANet \cite{han2021align}. Besides, the proposed TS-Conv is an anchor-free method, which is more flexible and does not rely on many hyperparameters of anchor boxes. The visualization results of TS-Conv on the DOTAv1.0 dataset \cite{xiaDOTALargeScaleDataset2018} are shown in Fig.~\ref{fig:11}. In addition, the performance of the lightweight model TS-Conv Lite (mAP$_{50}$=73.96) can reach the level of many larger models and has a detection speed that far exceeds that of other methods. Furthermore, the performance evaluation on the latest versions of the DOTA datasets, i.e., DOTAv1.5 and DOTAv2.0 \cite{li2020object} are listed in Table~\ref{table:7}. These datasets cover a wider category of objects and more small objects that are difficult to detect. The results also demonstrate the performance advantage of the proposed TS-Conv over existing methods.
\begin{table}[t]
	\centering
	\renewcommand\arraystretch{1}
	\setlength{\tabcolsep}{0.5mm}{
		\caption{\label{table:8}
			{Comparative performance of different methods on the HRSC2016 dataset}}
		\resizebox{0.48\textwidth}{!}{\setlength{\tabcolsep}{0.5mm}{
				\begin{tabular}{c|c|c|ccc}
					\hline\hline
					Method  & Anchor  & Backbone  & mAP$_{50}$(07) & mAP$_{50}$(12) & mAP$_{75}$(07) \\
					\hline
					R$^2$CNN \cite{jiang2017r2cnn}     & AB      & ResNet101 & 73.07   & 79.73   &-\\
					RoI-Transformer \cite{ding2019learning} & AB & ResNet101 & 86.20   & -      &- \\
					Gliding Vertex \cite{xu2020gliding}  & AB    & ResNet101 & 88.20   & -       &-\\
					BBAVectors \cite{yi2020oriented}  & AF     & ResNet101 & 88.60    & -       &-\\
					CenterMap OBB \cite{wang2020learning}  & AB  & ResNet50  & -       & 92.80   &- \\
					RetinaNet-R \cite{yang2019r3det}    & AB     & ResNet101 & 89.18   & 95.21  &- \\
					RetinaNet-GWD \cite{yang2021rethinking} & AB & ResNet50  & 85.56 & - & 60.31 \\ 
					RetinaNet-KLD \cite{yang2021learning} & AB & ResNet50  & 87.45 & - & 72.39 \\
					R$^3$Det \cite{yang2019r3det}     & AB       & ResNet101 & 89.26   & 96.01  &- \\
					R$^3$Det-DCL \cite{yang2021dense}   & AB     & ResNet101 & 89.46   & 96.41   &-\\
					R$^3$Det-GWD \cite{yang2021rethinking} & AB & ResNet50  & 89.43 & - & 68.88 \\
					R$^3$Det-KLD \cite{yang2021learning} & AB & ResNet50  & 89.97 & - & 77.38 \\
					S$^2$ANet \cite{han2021align}     & AB       & ResNet101 & 90.17   & 95.01   &-\\
					Oriented RepPoints \cite{li2022oriented} & AF & ResNet50  & 90.40   & 97.26   &- \\
					\hline
					GGHL \cite{huang2022general} (Baseline)    & AF   & DarkNet53 & 89.53  & 96.50 & 76.07 \\
					\textbf{TS-Conv}    & AF  & DarkNet53 & \textbf{90.59 \tiny{(+1.06)}}  & \textbf{97.64 \tiny{(+1.14)}}  &  \textbf{78.34 \tiny{(+2.27)}}\\
					\hline\hline
	\end{tabular}}}}\vspace{0.5em}
	\justifying{Note: Bold font indicates the best results. AF represents anchor-free methods, and AB represents anchor-based methods. The mAP$_{50}$(07) and mAP$_{50}$(12) represent the mAP calculated on standard of VOC07 and VOC12, respectively. Since the existing AOOD methods adopt different calculation standards, the mAPs obtained by them are all given here for fairness.}
\end{table}
\begin{table}[!t]
	\centering
	\renewcommand\arraystretch{1}
	\setlength{\tabcolsep}{0.5mm}{
		\caption{\label{table:9}
			{Comparative performance of different methods on the DIOR-R dataset}}
		\resizebox{0.48\textwidth}{!}{\setlength{\tabcolsep}{0.5mm}{
				\begin{threeparttable}	
					\begin{tabular}{c|c|c|ccc}
						\hline\hline
						Methods &  Anchor & Backbone & mAP$_{50}$  & mAP$_{75}$    & mAP$_{50:95}$     \\
						\hline
						RetinaNet-O \cite{linFocalLossDense2017}  & AB & ResNet50  & 57.55   & -    & -     \\
						Faster RCNN-O \cite{renFasterRCNNRealTime2017a}  & AB  & ResNet50  & 59.54    & -  & -      \\
						Gliding Vertex \cite{xu2020gliding} & AB  & ResNet50  & 60.06   & -    & -     \\
						RoI-Transformer \cite{ding2019learning}  & AB    & ResNet50   & 63.87      & -  & -    \\
						AOPG \cite{cheng2022anchor}   & AF   & ResNet50 & 64.41     & -    & -   \\
						Oriented RepPoints \cite{li2022oriented} & AF & ResNet50 & 66.71     & -    & -   \\
						\hline
						GGHL \cite{huang2022general} (Baseline) & AF  & DarkNet53 & 66.48  & 36.99    & 37.44      \\
						\textbf{TS-Conv} & AF & DarkNet53 & \textbf{68.47 \tiny{(+1.99)}} & \textbf{42.69 \tiny{(+5.70)}}& \textbf{41.38 \tiny{(+3.94)}} \\
						\hline\hline
					\end{tabular}
	\end{threeparttable}}}}\vspace{0.5em}
	\justifying{Note: Bold font indicates the best results. AF represents anchor-free methods, and AB represents anchor-based methods.}
\end{table}
\begin{table}[!t]
	\centering
	\renewcommand\arraystretch{1}
	\setlength{\tabcolsep}{1.2mm}{
		\caption{\label{table:10}
			{Comparative performance of different methods on the SSDD+ dataset}}
		\resizebox{0.48\textwidth}{!}{\setlength{\tabcolsep}{1.2mm}{
				\begin{threeparttable}
					\begin{tabular}{c|c|c|c|c|c}
						\hline\hline
						\multirow{2}{*}{Methods} & \multirow{2}{*}{Anchor} & \multirow{2}{*}{Backbone}& \multirow{2}{*}{mAP$_{30}$}  & \multirow{2}{*}{mAP$_{50}$} & \multirow{2}{*}{mAP$_{75}$} \\
						& &  &   & &  \\ \hline
						DRBox-v1 \cite{an2019drbox} \cite{wang2018simultaneous}  &  AB  & VGG16  & 86.41 & - & -   \\
						SDOE \cite{wang2018simultaneous}  &  AB  & VGG16 & -  & 82.40  & -   \\
						DRBox-v2 \cite{an2019drbox} & AB  & VGG16  & 92.81 & 85.17 & - \\\hline
						\begin{tabular}[c]{@{}c@{}}GGHL \cite{huang2022general} \\(Baseline1) \end{tabular}& AF  &  DarkNet53 & 95.10 & 90.22 & 22.18 \\						\cdashline{1-6}[0.8pt/2pt]
						\textbf{TS-Conv} & AF  &  DarkNet53 & \textbf{96.56 \tiny{(+1.46)}} & \textbf{92.48 \tiny{(+2.26)}} & \textbf{41.96 \tiny{(+19.78)}}  \\\hline
						\begin{tabular}[c]{@{}c@{}} LO-Det + GGHL \cite{huang2021lo} \\ (Baseline2)\end{tabular} & AF  & MobileNetv2  & 93.87 & 85.90 & 16.64 \\						\cdashline{1-6}[0.8pt/2pt]
						\textbf{LO-Det\cite{huang2021lo} + DTLA} & AF & MobileNetv2  & \textbf{93.89 \tiny{(+0.02)}} & \textbf{87.08 \tiny{(+1.18)}} & \textbf{26.73 \tiny{(+10.09)}} \\ 
						\hline\hline
					\end{tabular}
	\end{threeparttable}}}}\vspace{0.5em}
	\justifying{Note: The testing image size is 800 $\times$800 pixels. To be consistent with the comparison method, the confidence threshold is set to 0.2. AF represents anchor-free methods, and AB represents anchor-based methods.}
\end{table}
\begin{figure}[!t]
	\centering
	\epsfig{width=0.45\textwidth,file=12.pdf}
	\caption{Comparison of visualization results between GGHL and the proposed TS-Conv on the HRSC2016 dataset. Figs. (a-1)-(a-4) show the detection results of GGHL, and Figs. (b-1)-(b-4) show the detection results of TS-Conv.}\label{fig:12}
\end{figure}
\begin{figure}[!t]
	\centering
	\epsfig{width=0.45\textwidth,file=13.pdf}
	\caption{Visualization results of TS-Conv on the DIOR-R dataset.}\label{fig:13}
\end{figure}
\begin{figure}[!t]
	\centering
	\epsfig{width=0.43\textwidth,file=14.pdf}
	\caption{Presentation of other experiments. (a) Embedded edge devices, including Nvidia Jetson TX2, Nano and AGX Xavier, for evaluating the performance of lightweight models. (b) Visualization results of the proposed TS-Conv on the SSDD+ dataset.}\label{fig:14}
\end{figure}

\textbf{2) Comparison experiments on other datasets.} The results of comparison experiments on the HRSC2016 dataset are listed in Table~\ref{table:8}. TS-Conv also performs better than the existing methods in the ship detection, where the aspect ratio of objects is significant. Fig.~\ref{fig:12} shows that TS-Conv predicts more accurately and with fewer false alarms for oriented bounding boxes compared to GGHL \cite{huang2022general}. As shown in Table~\ref{table:9} and Fig.~\ref{fig:13}, TS-Conv also outperforms the existing methods on the DIOR-R dataset \cite{cheng2022anchor}, where objects have more scale variations and categories. In particular, the improvements are more significant for mAP$_{75}$ and mAP$_{50:95}$. The results on the SAR dataset SSDD+ are given in Table~\ref{table:10}. The results demonstrate that TS-Conv performs better on the datasets with other data modality. More visualized results are shown in Fig.~\ref{fig:14}. In addition, the experiments in Appendix C further demonstrate the generality of the proposed TS-Conv in other AOOD scenes. In summary, extensive comparison experiments are conducted on datasets covering multiple scenes, multimodal images (RGB, infrared, SAR, and panchromatic images), multiple categories of objects, and different lighting conditions (daytime and nighttime). The state-of-the-art results demonstrate the effectiveness and generality of TS-Conv.




